Multi-Dataset Co-Training with Sharpness-Aware Optimization for Audio Anti-spoofing

Audio anti-spoofing for automatic speaker verification aims to safeguard users' identities from spoofing attacks. Although state-of-the-art spoofing countermeasure(CM) models perform well on specific datasets, they lack generalization when evaluated with different datasets. To address this limitation, previous studies have explored large pre-trained models, which require significant resources and time. We aim to develop a compact but well-generalizing CM model that can compete with large pre-trained models. Our approach involves multi-dataset co-training and sharpness-aware minimization, which has not been investigated in this domain. Extensive experiments reveal that proposed method yield competitive results across various datasets while utilizing 4,000 times less parameters than the large pre-trained models.

==> tables/_AASIST.tex <==
\begin{table}[t]
  \caption{Results of AASIST model}
  \centering
  \label{tab:eer_types}
  \begin{tabularx}{\linewidth}{lccc}
    \toprule
    & \textbf{w/o SAM} & \textbf{SAM} & \textbf{ ASAM}\\
    \toprule
    %ASVspoof2015 (LA) & 38.83 & 29.50 &  - \\
    ASVspoof2019 (LA) & 1.15 &  - &  - \\
    \toprule
    ASVspoof2019 & - & - & -\\
    + ASVspoof2015 & & & \\
    \toprule
    ASVspoof2019 & - & - & -\\
    + ASVspoof2015  & & & \\
    + WaveFake & & & \\
    \bottomrule
  \end{tabularx}
\end{table}

==> tables/_InDomain.tex <==
\begin{table}[!t]
  \caption{In-domain evaluation results for ASVspoof2015, ASVspoof2019 LA. For model training, ASVspoof 2015, ASVspoof 2019 LA, and WaveFake are used and indicated as 2015, 2019 LA, and WaveFake. The results of the best performance are marked in boldface.}
  \centering
  \label{tab:in-domain}
  \begin{tabularx}{\linewidth}{lccc}
    \toprule
    Train dataset(s) & w/o SAM & SAM & ASAM \\
    \toprule
    \multicolumn{4}{c}{\textbf{ASVspoof 2015}}\\
    %& w/o SAM & SAM & ASAM \\
    \toprule
    2015 & 8.25 & 6.50 & 5.83 \\
    2019 LA & 5.98 & 4.32 & 3.53 \\
    2015 + 2019 LA & 0.69 & 0.80 & 0.83 \\
    2015 + 2019 LA + WaveFake & 0.82 & \textbf{0.66} & 1.82 \\
    \hline
    %\hline
    \multicolumn{4}{c}{\textbf{ASVspoof 2019}}\\
    \toprule
    %& w/o SAM & SAM & ASAM\\
    2015 LA & 38.83 & 29.50 & 30.70 \\
    2019 LA & 1.38 &  1.06 & 1.48 \\
    2015 LA+2019 LA &  1.56 & 1.07 & \textbf{0.99} \\
    2015 LA+2019 LA+WaveFake & 1.76 & 1.78 & 1.27 \\
    \bottomrule
  \end{tabularx}
  \vspace{-10pt}
\end{table}

==> tables/_OutOfDomain.tex <==
\begin{table}[!t]
  \caption{Out-of-domain evaluation results for ASVspoof2015, ASVspoof2019, and ASVspoof2021. For model training, ASVspoof 2015, ASVspoof 2019 LA, and WaveFake are used and indicated as 2015, 2019 LA, and WaveFake. The results of the top-2 performance are marked in boldface.}
  \centering
  \label{tab:out-of-domain}
  \begin{tabularx}{\linewidth}{lccc}
    \toprule
    Train dataset(s) & w/o SAM & SAM & ASAM \\
    \toprule
    \multicolumn{4}{c}{\textbf{ASVspoof 2021 LA}}\\
    \toprule
    %& w/o SAM & SAM & ASAM\\
    2015 LA & 39.87 & 32.27 & 31.09 \\
    2019 LA & 12.18 & \textbf{7.08} & 10.18 \\
    2015 LA+2019 LA & 12.25 & 12.52 & \textbf{9.37} \\
    2015 LA+2019 LA+WaveFake &  11.05 & 13.08 & 12.41 \\
    \toprule
    \multicolumn{4}{c}{\textbf{ASVspoof 2021 DF}}\\
    \toprule
    %& w/o SAM & SAM & ASAM\\
    2015 LA & 33.54 & 28.40 & 21.80 \\
    2019 LA & \textbf{18.20} & 21.16 & 19.58 \\
    2015 LA+2019 LA & 21.02 & 26.32 & 22.14 \\
    2015 LA+2019 LA+WaveFake &  19.76 & \textbf{19.49} & 19.84 \\
    \bottomrule
  \end{tabularx}
  \vspace{-10pt}
\end{table}
